Towards Micro-video Thumbnail Selection via a Multi-label Visual-semantic Embedding Model

The thumbnail, as the first sight of a micro-video, plays a pivotal role in attracting users to click and watch. While in the real scenario, the more the thumbnails satisfy the users, the more likely the micro-videos will be clicked. In this paper, we aim to select the thumbnail of a given micro-video that meets most users` interests. Towards this end, we present a multi-label visual-semantic embedding model to estimate the similarity between the pair of each frame and the popular topics that users are interested in. In this model, the visual and textual information is embedded into a shared semantic space, whereby the similarity can be measured directly, even the unseen words. Moreover, to compare the frame to all words from the popular topics, we devise an attention embedding space associated with the semantic-attention projection. With the help of these two embedding spaces, the popularity score of a frame, which is defined by the sum of similarity scores over the corresponding visual information and popular topic pairs, is achieved. Ultimately, we fuse the visual representation score and the popularity score of each frame to select the attractive thumbnail for the given micro-video. Extensive experiments conducted on a real-world dataset have well-verified that our model significantly outperforms several state-of-the-art baselines.

==> BIB/README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

IEEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> Data.tex <==
\section{DATA PREPARATION}
According to this, we detail the data preparation, including the auxiliary dataset, micro-video dataset construction, and popular topics collection.
\subsection{Auxiliary Dataset}
To train the deep transfer model, the auxiliary dataset should be large-scale, high-quality, and adaptive to our crossmodal multi-label similarity calculation. Overall, Open Images Dataset\footnote{http://storage.googleapis.com/openimages/web/index.html} is adopted as training dataset. It is a large-scale dataset with 9,011,219 images mainly collected from the Flickr\footnote{https://www.flickr.com/}, and each image is annotated with multiple labels over 600 categories. The labels cover the real-life entities and
are manually drawn by professional annotators to ensure the accuracy and consistency.
\subsection{Micro-video Dataset Construction}
To build the set of micro-videos, lack of the ground-truth of each micro-video still poses a big challenge. Previous studies choose the ground-truth thumbnails by some workers, but this strategy is inadaptive to our task. In our method, we suggest that the thumbnail is the frame whose content is largely related to the popular topics of the microvideo shared platform, yet the topics are affected by the realworld users’ interests which are probably different from those annotating workers’. Therefore, we collect the micro-videos with a large number of clicks to build the dataset and treat their posted thumbnails as the ground-truths. Because these posted thumbnails are the first sights of the micro-videos and convey the only information about the content. More clicks on the thumbnail mean it satisfies more users and is closer to the popular topics of the platform.

In practice, we collect some publishers and capture their posted micro-videos associated with the thumbnails. Since the aim is to obtain the micro-videos with a large number of
clicks, whose thumbnails are close to the popular topics, the influence of publishers themselves has to be eliminated. For this, we choose the publishers according to the number of their followers. As can be seen in Figure 4, the number of followers is limited to the range of 300-1000. Ultimately, we achieve 18,279 publishers to form the publishers set and crawl their micro-videos with more than 200 clicks.

To improve the performance of the thumbnail selection, some candidate frames are extracted from each micro-video based on visual quality and representativeness. Specifically, according to the findings [26], three types of low-quality frames would be detected and filtered out, including frames of dark, blurry, and uniform-colored. And we further filter out the near-duplicate frames via a clustering algorithm over the
high-quality frames. As shown in Figure 5, most micro-videos have 7-12 candidate frames. Although the posted thumbnail may not be contained in the set of candidate frames, we believe its nearest neighbor frame in the set is visually closer to the posted thumbnail. Statistically, the average similarity between the posted thumbnail and its nearest neighbor frame is about 93.8\%. Therefore, we take the nearest neighbor frames as the ground-truths for the micro-videos, instead of inserting the posted thumbnails into the sets of candidate frames. To verify the ground-truth, 1, 000 groups of candidate frames are randomly selected and annotated by 10 Instagram active users. From Figure 6, we observe that with the increasing number of clicks, the accuracy of manual labeling is improved. The number of clicks reflects the degree of attractiveness of the thumbnail to the users. Moreover, the accuracy can exceed 60\% in the worst case, proving that the ground-truth is more suitable than other frames as the thumbnail.
    \begin{figure}
	\centering
	  \includegraphics[width=0.4\textwidth]{Charts/figure4.png}
	  \vspace{-1mm}
	  \caption{Distribution of the number of followers in our dataset.}
	\label{fig_4}	  
	\vspace{-5mm}
\end{figure}

\subsection{Popular Topics Collection}

After the micro-video dataset collection and ground-truth construction, we focus on the popular topics collection. Therefore, about 1 million applicable comments are crawled
from Instagram to capture popular topics. Finally, we go through the entity words and obtain 111 high-frequency words to represent the popular topics. Table I lists a part of entity words and their frequencies.



==> IEEEtran/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> bak.tex <==
% by computing  users and items based on user intents, the similarities between their representations could be calculated to predict their interactions.  %interactions between them are predicted. 

% For this goal, leveraging the historical user-item interactions, we first construct the co-occurrence item graph,$\mathcal{G}=\{\mathbf{X}, \mathbf{A}\}$, in each modality to explore the user intent. 
% In particular, $\mathbf{x}_i\in \mathbf{X}$ represents the feature vector of $\text{v}_i$ and $\mathbf{A} \in \mathbb{R}^{M*M}$ reflects the connections between nodes and their neighbors, formally
% \begin{equation}
%     \mathbf{A}_{i, j} = 
%     \begin{cases}
%             1 &\  if\ \text{v}_j\ \in\ \mathcal{N}(\text{v}_i),\\
%             0 &\  if\ \text{v}_j\ \not\in\ \mathcal{N}(\text{v}_i),
%     \end{cases}
% \end{equation}
% where $\mathcal{N}(\text{v}_i)$ represents the neighbors of $\text{v}_i$.

% Towards this end, we suppose that user intents can be organized into $L$ levels from the fine-grained to the coarse-grained. 
% In the $l$-th level, there are $K^{(l)}$ user intents and the $k$-th one can be denoted as $\mathbf{c}^{(l)}_k$. 
% To model this multi-level relationships, leveraging the historical interactions between users and micro-videos, in each modality, we construct a item co-occurrence graph where an edge exists if two item nodes are co-interacted with several users.
% To learn the representations of these user intents, we construct the co-interacted item graph, 
% in which the presence of an edge signifies the corresponding item pair is consumed by some of same users. 
% To learn such multi-level user intents from users' historical behaviors, we construct the co-interacted item graph in each modality, where an edge exists if the item pair is co-interacted by several users in the historical records. 
% Let  $\mathcal{G}=\{\mathbf{X}, \mathbf{A}\}$ be the graph, where $\mathbf{X}\in\mathbb{R}^{M*D}$ and $\mathbf{A}\in\mathbb{R}^{M*M}$ denote the item feature matrix and adjacent matrix
% To be more specific, $\mathcal{G}=\{\mathbf{X}, \mathbf{A}\}$ denotes the graph, where $\mathbf{x}_i\in \mathbf{X}$ presents the feature vector of $\text{v}_i$ and $\mathbf{A} \in \mathbb{R}^{M*M}$ reflects the connections between the nodes and their neighbors. 
% $\mathbf{A}$ is formally defined as, 
% To learn the representations of these user intents, we construct the co-interacted item graph, $\mathcal{G}=\{\mathbf{X}, \mathbf{A}\}$ denotes the graph, where $\mathbf{x}_i\in \mathbf{X}$ presents the feature vector of $\text{v}_i$ and $\mathbf{A} \in \mathbb{R}^{M*M}$ reflects the connections between the nodes and their neighbors. 
